NNV: The Neural Network Verification Tool for Deep Neural Networks and Learning-Enabled Cyber-Physical Systems

This paper presents the Neural Network Verification (NNV) software tool, a set-based verification framework for deep neural networks (DNNs) and learning-enabled cyber-physical systems (CPS). The crux of NNV is a collection of reachability algorithms that make use of a variety of set representations, such as polyhedra, star sets, zonotopes, and abstract-domain representations. NNV supports both exact (sound and complete) and over-approximate (sound) reachability algorithms for verifying safety and robustness properties of feed-forward neural networks (FFNNs) with various activation functions. For learning-enabled CPS, such as closed-loop control systems incorporating neural networks, NNV provides exact and over-approximate reachability analysis schemes for linear plant models and FFNN controllers with piecewise-linear activation functions, such as ReLUs. For similar neural network control systems (NNCS) that instead have nonlinear plant models, NNV supports over-approximate analysis by combining the star set analysis used for FFNN controllers with zonotope-based analysis for nonlinear plant dynamics building on CORA. We evaluate NNV using two real-world case studies: the first is safety verification of ACAS Xu networks and the second deals with the safety verification of a deep learning-based adaptive cruise control system.

==> ACASXu_tab.tex <==

% \usepackage{multirow}
\begin{table}[tbp]
   \centering
   \resizebox{0.7\linewidth}{!}{
\begin{tabular}{|l|l|c|l|l|l|l|l|l|c|}
\hline
\multirow{2}{*}{\textbf{Prop.}} & \multirow{2}{*}{\textbf{ID}} & \multirow{2}{*}{\textbf{Result}} & \multicolumn{5}{c|}{\textbf{NNV}} & \textbf{Reluplex} & \multirow{2}{*}{\textbf{r}} \\ \cline{4-9}
 &  &  & $N_s$ & $N_r$ & $RT(sec)$ & $ST(sec)$ & $VT(sec)$ & $VT (sec)$ &  \\ \hline
  \multirow{3}{*}{$\phi_1$} & $N_{1\_1}$ & SAFE & 39811 & 316528 & 1546.99 & 21.12  & 1568.11  & 5986 & 3.81x \\ \cline{2-10}
  & $N_{1\_2}$ &  SAFE & 45606 & 454369 & 1829.22 & 23.2  & 1852.42  & 6477 & 3.5x \\ \cline{2-10}
  & $N_{1\_3}$ &  SAFE & 114219 & 1220251 & 4786.63 & 64.71  & 4851.34  & 54800 & 11.3x \\ \hline
 \multirow{6}{*}{$\phi_3$} & $N_{1\_3}$ &  SAFE & 12274 & 56745 & 221.33 & 7.15  & 228.48  & 1102 & 4.82x \\ \cline{2-10}
  & $N_{2\_1}$ &  SAFE & 16179 & 98566 & 202.43 & 8.89  & 211.32  & 1173 & 5.55x \\ \cline{2-10}
  & $N_{2\_2}$ &  SAFE & 6861 & 3619 & 91.34 & 4.35  & 95.69  & 634 & 6.63x \\ \cline{2-10}
  & $N_{2\_3}$ &  SAFE & 10614 & 54784 & 152.94 & 5.9  & 158.84  & 1014 & 6.4x \\ \cline{2-10}
  & $N_{5\_1}$ &  SAFE & 9461 & 82353 & 138.72 & 5.84  & 144.56  & 1097 & 7.59x \\ \cline{2-10}
  & $N_{5\_3}$ &  SAFE & 2874 & 17078 & 57.04 & 2.38  & 59.42  & 338 & 5.7x \\ \hline

  \multirow{11}{*}{$\phi_4$} & $N_{1\_1}$ &  SAFE & 14066 & 22794 & 88.04 & 7.82  & 95.86  & 653 & 14.49x \\ \cline{2-10}
  & $N_{1\_2}$ &  SAFE & 6082 & 36246 & 76.12 & 3.98  & 80.1  & 1424 & 17.78x \\ \cline{2-10}
  & $N_{1\_3}$ &  SAFE & 4456 & 18656 & 71.34 & 3.23  & 74.57  & 1294 & 17.35x \\ \cline{2-10}
  & $N_{1\_5}$ &  SAFE & 760  & 10061 & 30.94 & 1.34  & 32.28  & 393 & 12.17x \\ \cline{2-10}
  & $N_{2\_2}$ &  SAFE & 2391 & 15251 & 32.87 & 2.24  & 35.11  & 451 & 12.84x \\ \cline{2-10}
  & $N_{2\_3}$ &  SAFE & 2357 & 11577 & 32.26 & 2.15  & 34.41  & 293 & 8.52x \\ \cline{2-10}
  & $N_{2\_8}$ &  SAFE & 421 & 6058 & 26.12 & 1.01  & 27.13  & 653 & 24.1x \\ \cline{2-10}
  & $N_{3\_7}$ &  SAFE & 203 & 3616 & 14.01 & 0.72  & 14.73  & 357 & 24.24x \\ \cline{2-10}
 & $N_{3\_9}$ &  SAFE & 657 & 12662 & 36.9 & 1.22  & 38.12  & 715 & 18.75x \\ \cline{2-10}
 & $N_{5\_1}$ &  SAFE & 931 & 6010 & 18.9 & 1.3  & 20.2  & 585 & 28.96x \\ \cline{2-10}
 & $N_{4\_9}$ &  SAFE & 286 & 7849 & 25.9 & 0.79  & 26.69  & 489 & 18.3x \\ \hline
$\phi_5$ & $N_{1\_1}$ &  SAFE & 193080 & 1755370 & 6555.49 & 97.6  & 6653.09 & 20448 & 3.1x \\ \hline
$\phi_7$ & $N_{1\_9}$ &  TIMEOUT &  &  &  &  &  & TIMEOUT &  \\ \hline
$\phi_{10}$ & $N_{4\_5}$ &  SAFE & 41088 & 226122 & 1906.17 & 21.26  & 1927.43 & 23917 & 12.41x \\ \hline
\multicolumn{9}{|l|}{Average Improvement in Verification Time:} & $\approx$ 12.2x \\ \hline
\end{tabular}}
\caption{Safety verification results on ACAS Xu networks in which $N_s$ is the number of stars in the reachable set, $N_r$ is the number of stepReLU operations reduced, $RT$ is the reachable set computation time, $ST$ is the safety checking time, $VT = RT + ST$ is the total verification time, and $r$ is the ratio of the verification times between NNV and Reluplex.}
\label{tab:ACASXu}
\vspace{-1em}
\end{table}

==> Makefile <==

MAIN=main

all $(MAIN).pdf : $(MAIN).tex 
	pdflatex -halt-on-error $<
	-bibtex $(basename $<)
	pdflatex -halt-on-error $<
	pdflatex -halt-on-error $<

$(MAIN).fmt : prelude1.tex
	pdflatex -ini -jobname="$(MAIN)" "&pdflatex prelude1.tex\dump"

STEM=$(notdir $(PWD))

snapshot : $(MAIN).pdf
	@TODAY="`date +%Y%m%d`"; \
	N="1"; \
	while [ -f $$TODAY-$(STEM)-$$N.pdf ]; do \
	  N="`expr $$N + 1`"; done; \
	echo $(MAIN).pdf '->' $$TODAY-$(STEM)-$$N.pdf; \
	cp $(MAIN).pdf $$TODAY-$(STEM)-$$N.pdf

%.pdf : %.gpl
	gnuplot $(<)

plots : $(subst gpl,pdf,$(wildcard *.gpl))

clean :
	rm -f $(addprefix $(MAIN)., aux bbl blg fmt log out pdf)

.PHONY : plots snapshot clean



==> NNACC_tab_falsification.tex <==
\begin{table}[t!]
    \centering
   \resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{$\mathbf{x_{lead}(0)}$} & \multicolumn{2}{c|}{\textbf{Controller 1 (3 x 20)}} & \multicolumn{2}{c|}{\textbf{Controller 2 (5 x 20)}} & \multicolumn{2}{c|}{\textbf{Controller 3 (7 x 20)}} & \multicolumn{2}{c|}{\textbf{Controller 4 (10 x 20)}} \\ \cline{2-9}
 & \multicolumn{1}{c|}{$N_c$} & \multicolumn{1}{c|}{FT (sec)} & \multicolumn{1}{c|}{$N_c$} & \multicolumn{1}{c|}{FT (sec)} & \multicolumn{1}{c|}{$N_c$} & \multicolumn{1}{c|}{FT (sec)} & \multicolumn{1}{c|}{$N_c$} & \multicolumn{1}{c|}{FT (sec)} \\ \hline
[65, 70] & 100  & 43.63  & 303   & 45.25  & 486  & 46.91  & 134  & 49.13 \\ \hline
[70, 110] & 0  & 44.14  & 0     & 45.35  & 0    & 46.82  & 0    & 49.07 \\ \hline
\end{tabular}}
\caption{Falsification results for NNACC system with different neural network controllers using $1000$ random simulations in which $N_c$ is the number of counter examples and $FT$ is the falsification time.}
\label{tab:NNACC-falsification}
\vspace{-2em}
\end{table}

==> features.tex <==
\section{NNV's Features}


==> ncs_verifiers.tex <==
\begin{table}[]
  \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Approaches} & \textbf{Plant Dynamics} & \textbf{Discrete/Continuous} & \textbf{Activation Function} & \textbf{Size of Controller} \\ \hline
Polyhedron-based \cite{xx} & Linear & Discrete & ReLU & $\leq$ 100 neurons \\ \hline
Verisig \cite{xx} & Linear, Nonlinear & Discrete, Continuous & Sigmoid, Tanh & $\leq$ 50 neurons \\ \hline
SMC-based \cite{xx} & Linear & Discrete & ReLU & $\leq$ 200 neurons \\ \hline
Sherlock \cite{xx} & Linear, Nonlinear & Discrete, Continuous & ReLU & $\leq$ 500 neurons \\ \hline
Star-based & Linear, Nonlinear & Discrete, Continuous & ReLU & $\leq$ 200 neurons \\ \hline
\end{tabular}}
\caption{Approaches for neural network control systems verification in which the sizes of controllers are collected from the related experimental results.}
\label{tab:ncs-verifiers}
\end{table}

==> p1_p2_tab.tex <==
\begin{table}[]
\centering
\renewcommand{\arraystretch}{1.5}
\renewcommand{\tabcolsep}{1.5mm}
\begin{adjustbox}{angle=0, max width=\textwidth}
\begin{tabular}{c|ccccccccccc}
\hline
                              & \multicolumn{2}{c|}{\textbf{Reluplex}}                       & \multicolumn{2}{c|}{\textbf{Marabou}} & \multicolumn{2}{c|}{\textbf{Marabou DnC}} & \multicolumn{2}{c|}{\textbf{ReluVal}}                     & \multicolumn{3}{c}{\textbf{NNV Exact Star}}   \\ \cline{2-12} 
                              &  $VT$  & \multicolumn{1}{c|}{$V$}   &$VT$  & \multicolumn{1}{c|}{$V$}   & $VT$                & \multicolumn{1}{c|}{$V$}                 & $VT$                         & \multicolumn{1}{c|}{$V$}                        & $N_p$  & $VT$    & $V$   \\ \cline{2-12} 
\multirow{-3}{*}{\textbf{ID}} & \multicolumn{11}{c}{Property 1}                                                                                                                                                                                                                                                                                        \\ \hline
$N_{11}$                                              & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 1875}  & UNSAT & \cellcolor[HTML]{C7F7C7}410   & UNSAT & \cellcolor[HTML]{C7F7C7}74                  & UNSAT               & \cellcolor[HTML]{C7F7C7}0.08                         & UNSAT                      & 39810  & \cellcolor[HTML]{C7F7C7}5703  & UNSAT \\ 
$N_{12}$                                              & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 2697}  & UNSAT & \cellcolor[HTML]{C7F7C7}802   & UNSAT & \cellcolor[HTML]{C7F7C7}129                 & UNSAT               & \cellcolor[HTML]{C7F7C7}0.15                         & UNSAT                      & 45606  & \cellcolor[HTML]{C7F7C7}6869  & UNSAT \\ 
$N_{13}$                                              & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 25779} & UNSAT & \cellcolor[HTML]{C7F7C7}2319  & UNSAT & \cellcolor[HTML]{C7F7C7}1040                & UNSAT               & \cellcolor[HTML]{C7F7C7}1.30                         & UNSAT                      & 114219 & \cellcolor[HTML]{C7F7C7}19075 & UNSAT \\ 
$N_{14}$                                              & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 5953}  & UNSAT & \cellcolor[HTML]{C7F7C7}2326  & UNSAT & \cellcolor[HTML]{C7F7C7}948                 & UNSAT               & \cellcolor[HTML]{C7F7C7}1.35                         & UNSAT                      & 154449 & \cellcolor[HTML]{C7F7C7}23839 & UNSAT \\ 
$N_{15}$                                              & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 3825}  & UNSAT & \cellcolor[HTML]{C7F7C7}745   & UNSAT & \cellcolor[HTML]{C7F7C7}93                  & UNSAT               & \cellcolor[HTML]{C7F7C7}0.19                         & UNSAT                      & 122275 & \cellcolor[HTML]{C7F7C7}18615 & UNSAT \\ 
$N_{16}$                                              & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 2899}  & UNSAT & \cellcolor[HTML]{C7F7C7}1003  & UNSAT & \cellcolor[HTML]{C7F7C7}95                  & UNSAT               & \cellcolor[HTML]{C7F7C7}0.15                         & UNSAT                      & 0      & \cellcolor[HTML]{C7F7C7}0     & ERR   \\ 
$N_{17}$                                              & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 1061}  & UNSAT & \cellcolor[HTML]{C7F7C7}295   & UNSAT & \cellcolor[HTML]{C7F7C7}49                  & UNSAT               & \cellcolor[HTML]{C7F7C7}0.09                         & UNSAT                      & 66388  & \cellcolor[HTML]{C7F7C7}9007  & UNSAT \\ 
$N_{18}$                                              & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 3121}  & UNSAT & \cellcolor[HTML]{C7F7C7}209   & UNSAT & \cellcolor[HTML]{C7F7C7}45                  & UNSAT               & \cellcolor[HTML]{C7F7C7}0.07                         & UNSAT                      & 110085 & \cellcolor[HTML]{C7F7C7}16854 & UNSAT \\ 
$N_{19}$                                              & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 731}   & UNSAT & \cellcolor[HTML]{C7F7C7}116   & UNSAT & \cellcolor[HTML]{C7F7C7}33                  & UNSAT               & \cellcolor[HTML]{C7F7C7}0.07                         & UNSAT                      & 135559 & \cellcolor[HTML]{C7F7C7}19274 & UNSAT \\ \hline
                                                      & \multicolumn{11}{c}{Property 2}                                                                                                                                                                                                                                                                                        \\ \hline
$N_{11}$                                              & \cellcolor[HTML]{C7F7C7}4888                         & UNSAT & \cellcolor[HTML]{C7F7C7}4290  & UNSAT & \cellcolor[HTML]{C7F7C7}1887                & UNSAT               & {\cellcolor[HTML]{C7F7C7}0.55}    & {UNSAT} & 39810  & \cellcolor[HTML]{C7F7C7}10    & UNSAT \\ 
$N_{12}$                                              & \cellcolor[HTML]{C7F7C7}396                          & SAT   & \cellcolor[HTML]{C7F7C7}760   & SAT   & \cellcolor[HTML]{C7F7C7}450                 & SAT                 & {\cellcolor[HTML]{C7F7C7}15.51}   & {SAT}   & 45606  & \cellcolor[HTML]{C7F7C7}11    & SAT   \\ 
$N_{13}$                                              & \cellcolor[HTML]{C7F7C7}1704                         & SAT   & \cellcolor[HTML]{C7F7C7}1122  & SAT   & \cellcolor[HTML]{C7F7C7}5015                & SAT                 & {\cellcolor[HTML]{C7F7C7}12.60}   & {SAT}   & 114219 & \cellcolor[HTML]{C7F7C7}28    & SAT   \\ 
$N_{14}$                                              & \cellcolor[HTML]{C7F7C7}881                          & SAT   & \cellcolor[HTML]{C7F7C7}56    & SAT   & \cellcolor[HTML]{C7F7C7}4028                & SAT                 & {\cellcolor[HTML]{C7F7C7}3.43}    & {SAT}   & 154449 & \cellcolor[HTML]{C7F7C7}38    & SAT   \\ 
$N_{15}$                                              & \cellcolor[HTML]{C7F7C7}22                           & SAT   & \cellcolor[HTML]{C7F7C7}737   & SAT   & \cellcolor[HTML]{C7F7C7}230                 & SAT                 & {\cellcolor[HTML]{C7F7C7}1004.93} & {SAT}   & 122275 & \cellcolor[HTML]{C7F7C7}30    & SAT   \\ 
$N_{16}$                                              & \cellcolor[HTML]{C7F7C7}242                          & SAT   & \cellcolor[HTML]{C7F7C7}5493  & SAT   & \cellcolor[HTML]{C7F7C7}961                 & SAT                 & {\cellcolor[HTML]{C7F7C7}33.14}   & {ERR}   & 0      & \cellcolor[HTML]{C7F7C7}0     & ERR   \\ 
$N_{17}$                                              & \cellcolor[HTML]{C7F7C7}4759                         & UNSAT & \cellcolor[HTML]{C7F7C7}9585  & UNSAT & \cellcolor[HTML]{C7F7C7}2847                & UNSAT               & {\cellcolor[HTML]{C7F7C7}5.14}    & {UNSAT} & 66388  & \cellcolor[HTML]{C7F7C7}16    & UNSAT \\ 
$N_{18}$                                              & \cellcolor[HTML]{C7F7C7}15180                        & UNSAT & \cellcolor[HTML]{C7F7C7}26824 & UNSAT & \cellcolor[HTML]{C7F7C7}13095               & UNSAT               & {\cellcolor[HTML]{C7F7C7}20.63}   & {UNSAT} & 110085 & \cellcolor[HTML]{C7F7C7}27    & UNSAT \\ 
$N_{19}$                                              & \cellcolor[HTML]{C7F7C7}8211                         & UNSAT & \cellcolor[HTML]{C7F7C7}16207 & UNSAT & \cellcolor[HTML]{C7F7C7}5905                & UNSAT               & {\cellcolor[HTML]{C7F7C7}9.05}    & {UNSAT} & 135559 & \cellcolor[HTML]{C7F7C7}34    & UNSAT \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> p3_tab.tex <==
\begin{table}
\centering
\renewcommand{\arraystretch}{1.5}
\renewcommand{\tabcolsep}{1.5mm}
\begin{adjustbox}{angle=0, max width=\textwidth}
\begin{tabular}{c|ccccccccccccccccc}
\hline
                              & \multicolumn{2}{c|}{\textbf{Zonotope}} & \multicolumn{2}{c|}{\textbf{Abstract Domain}} & \multicolumn{2}{c|}{\textbf{Reluplex}} & \multicolumn{2}{c|}{\textbf{Marabou}} & \multicolumn{2}{c|}{\textbf{Marabou DnC}} & \multicolumn{2}{c|}{\textbf{ReluVal}} & \multicolumn{3}{c|}{\textbf{NNV Exact Star}} & \multicolumn{2}{c}{\textbf{NNV Appr. Star}} \\ \cline{2-18} 
\multirow{-2}{*}{\textbf{ID}} &  $VT$  & \multicolumn{1}{c|}{$V$}    & $VT$                              &\multicolumn{1}{c|}{$V$}       &  $VT$  & \multicolumn{1}{c|}{$V$}    & $VT$                          & \multicolumn{1}{c|}{$V$}   & $VT$                            & \multicolumn{1}{c|}{$V$}   & $VT$                            & \multicolumn{1}{c|}{$V$}  & $N_p$ &  $VT$ & \multicolumn{1}{c|}{$V$}   &  $VT$     & \multicolumn{1}{c}{$V$}       \\ \hline
$N_{11}$                      & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}1.96      & UNSAT     & \cellcolor[HTML]{C7F7C7}6156  & UNSAT  & \cellcolor[HTML]{C7F7C7}3637  & UNSAT & \cellcolor[HTML]{C7F7C7}73560   & UNSAT  &\cellcolor[HTML]{C7F7C7}96.83   & UNSAT   & \cellcolor[HTML]{FFFFC7}70631 & \cellcolor[HTML]{C7F7C7}1463  & UNSAT & \cellcolor[HTML]{C7F7C7}1.89     & UNK       \\ 
$N_{12}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}2.31      & UNSAT     & \cellcolor[HTML]{C7F7C7}4942  & UNSAT  & \cellcolor[HTML]{C7F7C7}3418  & UNSAT & \cellcolor[HTML]{C7F7C7}3221    & UNSAT  &\cellcolor[HTML]{C7F7C7}1.87   & UNSAT    & \cellcolor[HTML]{FFFFC7}39529 & \cellcolor[HTML]{C7F7C7}1026 & UNSAT & \cellcolor[HTML]{C7F7C7}1.86     & UNK       \\ 
$N_{13}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}2.42      & UNSAT     & \cellcolor[HTML]{C7F7C7}1134  & UNSAT  & \cellcolor[HTML]{C7F7C7}1795  & UNSAT & \cellcolor[HTML]{C7F7C7}10858   & UNSAT  &\cellcolor[HTML]{C7F7C7}3.22   & UNSAT    & \cellcolor[HTML]{FFFFC7}12274 & \cellcolor[HTML]{C7F7C7}299  & UNSAT & \cellcolor[HTML]{C7F7C7}2.16     & UNK       \\ 
$N_{14}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.73      & UNK       & \cellcolor[HTML]{C7F7C7}528   & UNSAT  & \cellcolor[HTML]{C7F7C7}187   & UNSAT & \cellcolor[HTML]{C7F7C7}186     & UNSAT  &\cellcolor[HTML]{C7F7C7}0.27   & UNSAT    & \cellcolor[HTML]{FFFFC7}4275  & \cellcolor[HTML]{C7F7C7}52   & UNSAT & \cellcolor[HTML]{C7F7C7}1.04     & UNSAT     \\ 
$N_{15}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}1.68      & UNK       & \cellcolor[HTML]{C7F7C7}317   & UNSAT  & \cellcolor[HTML]{C7F7C7}124   & UNSAT & \cellcolor[HTML]{C7F7C7}193     & UNSAT  &\cellcolor[HTML]{C7F7C7}0.11   & UNSAT    & \cellcolor[HTML]{FFFFC7}4744  & \cellcolor[HTML]{C7F7C7}84   & UNSAT & \cellcolor[HTML]{C7F7C7}0.96     & UNSAT     \\ 
$N_{16}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.99      & UNSAT     & \cellcolor[HTML]{C7F7C7}64    & UNSAT  & \cellcolor[HTML]{C7F7C7}37    & UNSAT & \cellcolor[HTML]{C7F7C7}23      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.04   & UNSAT     & \cellcolor[HTML]{FFFFC7}1266  & \cellcolor[HTML]{C7F7C7}20   & UNSAT & \cellcolor[HTML]{C7F7C7}0.79     & UNSAT     \\ 
$N_{17}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}0.73      & UNK       & \cellcolor[HTML]{C7F7C7}1     & SAT    & \cellcolor[HTML]{C7F7C7}5     & SAT   & \cellcolor[HTML]{C7F7C7}6       & SAT    &\cellcolor[HTML]{C7F7C7}0.03   &SAT    & \cellcolor[HTML]{FFFFC7}500   & \cellcolor[HTML]{C7F7C7}6    & SAT   & \cellcolor[HTML]{C7F7C7}0.64     & UNK       \\ 
$N_{18}$                      & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}0.62      & UNK       & \cellcolor[HTML]{C7F7C7}3     & SAT    & \cellcolor[HTML]{C7F7C7}2     & SAT   & \cellcolor[HTML]{C7F7C7}6       & SAT    &\cellcolor[HTML]{C7F7C7}0.03   &SAT    & \cellcolor[HTML]{FFFFC7}393   & \cellcolor[HTML]{C7F7C7}5    & SAT   & \cellcolor[HTML]{C7F7C7}0.45     & UNK       \\ 
$N_{19}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.52      & UNK       & \cellcolor[HTML]{C7F7C7}2     & SAT    & \cellcolor[HTML]{C7F7C7}2     & SAT   & \cellcolor[HTML]{C7F7C7}6       & SAT    &\cellcolor[HTML]{C7F7C7}0.03   &SAT    & \cellcolor[HTML]{FFFFC7}290   & \cellcolor[HTML]{C7F7C7}3    & SAT   & \cellcolor[HTML]{C7F7C7}0.42     & UNK       \\ 
$N_{21}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}2.36      & UNK       & \cellcolor[HTML]{C7F7C7}1208  & UNSAT  & \cellcolor[HTML]{C7F7C7}1001  & UNSAT & \cellcolor[HTML]{C7F7C7}813     & UNSAT  &\cellcolor[HTML]{C7F7C7}18.46   & UNSAT    & \cellcolor[HTML]{FFFFC7}16179 & \cellcolor[HTML]{C7F7C7}336  & UNSAT & \cellcolor[HTML]{C7F7C7}1.79     & UNK       \\ 
$N_{22}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.64      & UNK       & \cellcolor[HTML]{C7F7C7}653   & UNSAT  & \cellcolor[HTML]{C7F7C7}480   & UNSAT & \cellcolor[HTML]{C7F7C7}2106    & UNSAT  &\cellcolor[HTML]{C7F7C7}7.22   & UNSAT    & \cellcolor[HTML]{FFFFC7}6861  & \cellcolor[HTML]{C7F7C7}126  & UNSAT & \cellcolor[HTML]{C7F7C7}1.39     & UNK       \\ 
$N_{23}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.93      & UNK       & \cellcolor[HTML]{C7F7C7}1043  & UNSAT  & \cellcolor[HTML]{C7F7C7}1103  & UNSAT & \cellcolor[HTML]{C7F7C7}1163    & UNSAT  &\cellcolor[HTML]{C7F7C7}2.73   &UNSAT    & \cellcolor[HTML]{FFFFC7}10614 & \cellcolor[HTML]{C7F7C7}203  & UNSAT & \cellcolor[HTML]{C7F7C7}1.69     & UNK       \\ 
$N_{24}$                      & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}1.01      & UNSAT     & \cellcolor[HTML]{C7F7C7}41    & UNSAT  & \cellcolor[HTML]{C7F7C7}22    & UNSAT & \cellcolor[HTML]{C7F7C7}8      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.48   &UNSAT    & \cellcolor[HTML]{FFFFC7}345   & \cellcolor[HTML]{C7F7C7}5    & UNSAT & \cellcolor[HTML]{C7F7C7}0.55     & UNSAT     \\ 
$N_{25}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.82      & UNK       & \cellcolor[HTML]{C7F7C7}235   & UNSAT  & \cellcolor[HTML]{C7F7C7}58    & UNSAT & \cellcolor[HTML]{C7F7C7}13      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.31   &UNSAT   & \cellcolor[HTML]{FFFFC7}2456  & \cellcolor[HTML]{C7F7C7}34   & UNSAT & \cellcolor[HTML]{C7F7C7}1.17     & UNSAT     \\ 
$N_{26}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}0.82      & UNSAT     & \cellcolor[HTML]{C7F7C7}79    & UNSAT  & \cellcolor[HTML]{C7F7C7}23    & UNSAT & \cellcolor[HTML]{C7F7C7}8      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.03   &UNSAT    & \cellcolor[HTML]{FFFFC7}253   & \cellcolor[HTML]{C7F7C7}4    & UNSAT & \cellcolor[HTML]{C7F7C7}0.69     & UNSAT     \\ 
$N_{27}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.53      & UNSAT     & \cellcolor[HTML]{C7F7C7}116   & UNSAT  & \cellcolor[HTML]{C7F7C7}57    & UNSAT & \cellcolor[HTML]{C7F7C7}9      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.20   &UNSAT    & \cellcolor[HTML]{FFFFC7}1199  & \cellcolor[HTML]{C7F7C7}17   & UNSAT & \cellcolor[HTML]{C7F7C7}1.01     & UNSAT     \\ 
$N_{28}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.03      & UNSAT     & \cellcolor[HTML]{C7F7C7}83    & UNSAT  & \cellcolor[HTML]{C7F7C7}13    & UNSAT & \cellcolor[HTML]{C7F7C7}8      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.04   &UNSAT    & \cellcolor[HTML]{FFFFC7}326   & \cellcolor[HTML]{C7F7C7}5    & UNSAT & \cellcolor[HTML]{C7F7C7}0.50     & UNSAT     \\ 
$N_{29}$                      & \cellcolor[HTML]{C7F7C7}0.05  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.38      & UNSAT     & \cellcolor[HTML]{C7F7C7}27    & UNSAT  & \cellcolor[HTML]{C7F7C7}2     & UNSAT & \cellcolor[HTML]{C7F7C7}7      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.01   &UNSAT    & \cellcolor[HTML]{FFFFC7}188   & \cellcolor[HTML]{C7F7C7}2    & UNSAT & \cellcolor[HTML]{C7F7C7}0.36     & UNSAT     \\ 
$N_{31}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}2.41      & UNSAT     & \cellcolor[HTML]{C7F7C7}177   & UNSAT  & \cellcolor[HTML]{C7F7C7}97    & UNSAT & \cellcolor[HTML]{C7F7C7}240     & UNSAT  &\cellcolor[HTML]{C7F7C7}2.58   &UNSAT    & \cellcolor[HTML]{FFFFC7}5967  & \cellcolor[HTML]{C7F7C7}118  & UNSAT & \cellcolor[HTML]{C7F7C7}1.13     & UNSAT     \\ 
$N_{32}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}2.32      & UNK       & \cellcolor[HTML]{C7F7C7}1561  & UNSAT  & \cellcolor[HTML]{C7F7C7}1973  & UNSAT & \cellcolor[HTML]{C7F7C7}1564    & UNSAT  &\cellcolor[HTML]{C7F7C7}5.27   &UNSAT    & \cellcolor[HTML]{FFFFC7}36967 & \cellcolor[HTML]{C7F7C7}907  & UNSAT & \cellcolor[HTML]{C7F7C7}1.91     & UNK       \\ 
$N_{33}$                      & \cellcolor[HTML]{C7F7C7}0.08  & UNK    & \cellcolor[HTML]{C7F7C7}2.09      & UNSAT     & \cellcolor[HTML]{C7F7C7}1105  & UNSAT  & \cellcolor[HTML]{C7F7C7}344   & UNSAT & \cellcolor[HTML]{C7F7C7}891     & UNSAT  &\cellcolor[HTML]{C7F7C7}0.26   &UNSAT    & \cellcolor[HTML]{FFFFC7}7848  & \cellcolor[HTML]{C7F7C7}193  & UNSAT & \cellcolor[HTML]{C7F7C7}1.76     & UNSAT     \\ 
$N_{34}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}2.89      & UNK       & \cellcolor[HTML]{C7F7C7}209   & UNSAT  & \cellcolor[HTML]{C7F7C7}106   & UNSAT & \cellcolor[HTML]{C7F7C7}34      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.49   &UNSAT    & \cellcolor[HTML]{FFFFC7}2077  & \cellcolor[HTML]{C7F7C7}46   & UNSAT & \cellcolor[HTML]{C7F7C7}1.96     & UNK       \\ 
$N_{35}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.50      & UNK       & \cellcolor[HTML]{C7F7C7}83    & UNSAT  & \cellcolor[HTML]{C7F7C7}41    & UNSAT & \cellcolor[HTML]{C7F7C7}10      & UNSAT  &\cellcolor[HTML]{C7F7C7}5.01   &UNSAT    & \cellcolor[HTML]{FFFFC7}1034  & \cellcolor[HTML]{C7F7C7}16   & UNSAT & \cellcolor[HTML]{C7F7C7}1.16     & UNSAT     \\ 
$N_{36}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}2.50      & UNK       & \cellcolor[HTML]{C7F7C7}255   & UNSAT  & \cellcolor[HTML]{C7F7C7}120   & UNSAT & \cellcolor[HTML]{C7F7C7}194     & UNSAT  &\cellcolor[HTML]{C7F7C7}138.73   &UNSAT    & \cellcolor[HTML]{FFFFC7}1857  & \cellcolor[HTML]{C7F7C7}37   & UNSAT & \cellcolor[HTML]{C7F7C7}1.86     & UNK       \\ 
$N_{37}$                      & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}0.76      & UNSAT     & \cellcolor[HTML]{C7F7C7}35    & UNSAT  & \cellcolor[HTML]{C7F7C7}8     & UNSAT & \cellcolor[HTML]{C7F7C7}7      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.10   &UNSAT    & \cellcolor[HTML]{FFFFC7}107   & \cellcolor[HTML]{C7F7C7}2    & UNSAT & \cellcolor[HTML]{C7F7C7}0.56     & UNSAT     \\ 
$N_{38}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}1.34      & UNK       & \cellcolor[HTML]{C7F7C7}179   & UNSAT  & \cellcolor[HTML]{C7F7C7}57    & UNSAT & \cellcolor[HTML]{C7F7C7}25      & UNSAT  &\cellcolor[HTML]{C7F7C7}3.51   &UNSAT    & \cellcolor[HTML]{FFFFC7}654   & \cellcolor[HTML]{C7F7C7}10   & UNSAT & \cellcolor[HTML]{C7F7C7}1.04     & UNSAT     \\ 
$N_{39}$                      & \cellcolor[HTML]{C7F7C7}0.08  & UNK    & \cellcolor[HTML]{C7F7C7}1.54      & UNK       & \cellcolor[HTML]{C7F7C7}118   & UNSAT  & \cellcolor[HTML]{C7F7C7}55    & UNSAT & \cellcolor[HTML]{C7F7C7}35      & UNSAT  &\cellcolor[HTML]{C7F7C7}2.36   &UNSAT    & \cellcolor[HTML]{FFFFC7}1201  & \cellcolor[HTML]{C7F7C7}21   & UNSAT & \cellcolor[HTML]{C7F7C7}0.75     & UNSAT     \\ 
$N_{41}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}1.34      & UNK       & \cellcolor[HTML]{C7F7C7}201   & UNSAT  & \cellcolor[HTML]{C7F7C7}94    & UNSAT & \cellcolor[HTML]{C7F7C7}914     & UNSAT  &\cellcolor[HTML]{C7F7C7}7.29   &UNSAT    & \cellcolor[HTML]{FFFFC7}2276  & \cellcolor[HTML]{C7F7C7}43   & UNSAT & \cellcolor[HTML]{C7F7C7}1.20     & UNK       \\ 
$N_{42}$                      & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}2.13      & UNK       & \cellcolor[HTML]{C7F7C7}2882  & UNSAT  & \cellcolor[HTML]{C7F7C7}1724  & UNSAT & \cellcolor[HTML]{C7F7C7}11861   & UNSAT  &\cellcolor[HTML]{C7F7C7}90.93   &UNSAT    & \cellcolor[HTML]{FFFFC7}17894 & \cellcolor[HTML]{C7F7C7}444  & UNSAT & \cellcolor[HTML]{C7F7C7}1.67     & UNK       \\ 
$N_{43}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}2.05      & UNK       & \cellcolor[HTML]{C7F7C7}1767  & UNSAT  & \cellcolor[HTML]{C7F7C7}1257  & UNSAT & \cellcolor[HTML]{C7F7C7}1014    & UNSAT  &\cellcolor[HTML]{C7F7C7}2.13   &UNSAT    & \cellcolor[HTML]{FFFFC7}20746 & \cellcolor[HTML]{C7F7C7}618  & UNSAT & \cellcolor[HTML]{C7F7C7}1.79     & UNK       \\ 
$N_{44}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}1.51      & UNK       & \cellcolor[HTML]{C7F7C7}86    & UNSAT  & \cellcolor[HTML]{C7F7C7}19    & UNSAT & \cellcolor[HTML]{C7F7C7}8      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.11   &UNSAT    & \cellcolor[HTML]{FFFFC7}560   & \cellcolor[HTML]{C7F7C7}8    & UNSAT & \cellcolor[HTML]{C7F7C7}0.94     & UNSAT     \\ 
$N_{45}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.90      & UNSAT     & \cellcolor[HTML]{C7F7C7}35    & UNSAT  & \cellcolor[HTML]{C7F7C7}14    & UNSAT & \cellcolor[HTML]{C7F7C7}8      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.09   &UNSAT    & \cellcolor[HTML]{FFFFC7}351   & \cellcolor[HTML]{C7F7C7}4    & UNSAT & \cellcolor[HTML]{C7F7C7}0.77     & UNSAT     \\ 
$N_{46}$                      & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}2.78      & UNSAT     & \cellcolor[HTML]{C7F7C7}300   & UNSAT  & \cellcolor[HTML]{C7F7C7}118   & UNSAT & \cellcolor[HTML]{C7F7C7}55      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.14   &UNSAT    & \cellcolor[HTML]{FFFFC7}2496  & \cellcolor[HTML]{C7F7C7}61   & UNSAT & \cellcolor[HTML]{C7F7C7}2.60     & UNSAT     \\ 
$N_{47}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.45      & UNK       & \cellcolor[HTML]{C7F7C7}126   & UNSAT  & \cellcolor[HTML]{C7F7C7}54    & UNSAT & \cellcolor[HTML]{C7F7C7}43      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.52   &UNSAT    & \cellcolor[HTML]{FFFFC7}944   & \cellcolor[HTML]{C7F7C7}13   & UNSAT & \cellcolor[HTML]{C7F7C7}0.70     & UNSAT     \\ 
$N_{48}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}1.33      & UNSAT     & \cellcolor[HTML]{C7F7C7}142   & UNSAT  & \cellcolor[HTML]{C7F7C7}36    & UNSAT & \cellcolor[HTML]{C7F7C7}41      & UNSAT  &\cellcolor[HTML]{C7F7C7}1.65   &UNSAT    & \cellcolor[HTML]{FFFFC7}576   & \cellcolor[HTML]{C7F7C7}9    & UNSAT & \cellcolor[HTML]{C7F7C7}0.81     & UNSAT     \\ 
$N_{49}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}2.41      & UNSAT     & \cellcolor[HTML]{C7F7C7}143   & UNSAT  & \cellcolor[HTML]{C7F7C7}33    & UNSAT & \cellcolor[HTML]{C7F7C7}22      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.07   &UNSAT    & \cellcolor[HTML]{FFFFC7}611   & \cellcolor[HTML]{C7F7C7}19   & UNSAT & \cellcolor[HTML]{C7F7C7}1.02     & UNSAT     \\ 
$N_{51}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.65      & UNK       & \cellcolor[HTML]{C7F7C7}1131  & UNSAT  & \cellcolor[HTML]{C7F7C7}764   & UNSAT & \cellcolor[HTML]{C7F7C7}1910    & UNSAT  &\cellcolor[HTML]{C7F7C7}19.33   &UNSAT    & \cellcolor[HTML]{FFFFC7}9461  & \cellcolor[HTML]{C7F7C7}180  & UNSAT & \cellcolor[HTML]{C7F7C7}1.47     & UNK       \\ 
$N_{52}$                      & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}1.15      & UNK       & \cellcolor[HTML]{C7F7C7}151   & UNSAT  & \cellcolor[HTML]{C7F7C7}120   & UNSAT & \cellcolor[HTML]{C7F7C7}635     & UNSAT  &\cellcolor[HTML]{C7F7C7}1.94   &UNSAT    & \cellcolor[HTML]{FFFFC7}2104  & \cellcolor[HTML]{C7F7C7}40   & UNSAT & \cellcolor[HTML]{C7F7C7}1.01     & UNSAT     \\ 
$N_{53}$                      & \cellcolor[HTML]{C7F7C7}0.17  & UNK    & \cellcolor[HTML]{C7F7C7}1.73      & UNSAT     & \cellcolor[HTML]{C7F7C7}341   & UNSAT  & \cellcolor[HTML]{C7F7C7}146   & UNSAT & \cellcolor[HTML]{C7F7C7}64     & UNSAT  &\cellcolor[HTML]{C7F7C7}0.13   &UNSAT    & \cellcolor[HTML]{FFFFC7}2874  & \cellcolor[HTML]{C7F7C7}41   & UNSAT & \cellcolor[HTML]{C7F7C7}1.41     & UNSAT     \\ 
$N_{54}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.53      & UNK       & \cellcolor[HTML]{C7F7C7}62    & UNSAT  & \cellcolor[HTML]{C7F7C7}42    & UNSAT & \cellcolor[HTML]{C7F7C7}10      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.13   &UNSAT    & \cellcolor[HTML]{FFFFC7}758   & \cellcolor[HTML]{C7F7C7}13   & UNSAT & \cellcolor[HTML]{C7F7C7}1.06     & UNSAT     \\ 
$N_{55}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}1.83      & UNK       & \cellcolor[HTML]{C7F7C7}86    & UNSAT  & \cellcolor[HTML]{C7F7C7}27    & UNSAT & \cellcolor[HTML]{C7F7C7}18      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.41   &UNSAT    & \cellcolor[HTML]{FFFFC7}1305  & \cellcolor[HTML]{C7F7C7}19   & UNSAT & \cellcolor[HTML]{C7F7C7}1.06     & UNSAT     \\ 
$N_{56}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}2.14      & UNK       & \cellcolor[HTML]{C7F7C7}283   & UNSAT  & \cellcolor[HTML]{C7F7C7}81    & UNSAT & \cellcolor[HTML]{C7F7C7}47      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.86   &UNSAT    & \cellcolor[HTML]{FFFFC7}1143  & \cellcolor[HTML]{C7F7C7}21   & UNSAT & \cellcolor[HTML]{C7F7C7}1.12     & UNSAT     \\ 
$N_{57}$                      & \cellcolor[HTML]{C7F7C7}0.07  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.43      & UNSAT     & \cellcolor[HTML]{C7F7C7}35    & UNSAT  & \cellcolor[HTML]{C7F7C7}5     & UNSAT & \cellcolor[HTML]{C7F7C7}8      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.02   &UNSAT    & \cellcolor[HTML]{FFFFC7}88    & \cellcolor[HTML]{C7F7C7}1    & UNSAT & \cellcolor[HTML]{C7F7C7}0.34     & UNSAT     \\ 
$N_{58}$                      & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}1.58      & UNSAT     & \cellcolor[HTML]{C7F7C7}310   & UNSAT  & \cellcolor[HTML]{C7F7C7}157   & UNSAT & \cellcolor[HTML]{C7F7C7}22      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.06   &UNSAT    & \cellcolor[HTML]{FFFFC7}2368  & \cellcolor[HTML]{C7F7C7}42   & UNSAT & \cellcolor[HTML]{C7F7C7}0.92     & UNSAT     \\ 
$N_{59}$                      & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.72      & UNK       & \cellcolor[HTML]{C7F7C7}19    & UNSAT  & \cellcolor[HTML]{C7F7C7}8     & UNSAT & \cellcolor[HTML]{C7F7C7}8      & UNSAT  &\cellcolor[HTML]{C7F7C7}0.07   &UNSAT    & \cellcolor[HTML]{FFFFC7}107   & \cellcolor[HTML]{C7F7C7}3    & UNSAT & \cellcolor[HTML]{C7F7C7}0.58     & UNSAT     \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}

==> p4_tab.tex <==
\begin{table}
\centering
\renewcommand{\arraystretch}{1.5}
\renewcommand{\tabcolsep}{1.5mm}
\begin{adjustbox}{angle=0, max width=\textwidth}
\begin{tabular}{c|ccccccccccccccccc}
\hline
                               & \multicolumn{2}{c|}{\textbf{Zonotope}} & \multicolumn{2}{c|}{\textbf{Abstract}} & \multicolumn{2}{c|}{\textbf{Reluplex}}                      & \multicolumn{2}{c|}{\textbf{Marabou}} & \multicolumn{2}{c|}{\textbf{Marabou DnC}} & \multicolumn{2}{c|}{ \textbf{ReluVal}} & \multicolumn{3}{c|}{\textbf{NNV Exact Star}} & \multicolumn{2}{c}{\textbf{NNV Appr. Star}} \\ \cline{2-18} 
\multirow{-2}{*}{\textbf{ID}} &  $VT$  & \multicolumn{1}{c|}{$V$}    & $VT$                              &\multicolumn{1}{c|}{$V$}       &  $VT$  & \multicolumn{1}{c|}{$V$}    & $VT$                          & \multicolumn{1}{c|}{$V$}   & $VT$                            & \multicolumn{1}{c|}{$V$}   & $VT$                            & \multicolumn{1}{c|}{$V$}  & $N_p$ &  $VT$ & \multicolumn{1}{c|}{$V$}   &  $VT$     & \multicolumn{1}{c}{$V$}       \\ \hline
$N_{11}$                                              & \cellcolor[HTML]{C7F7C7}0.10  & UNK    & \cellcolor[HTML]{C7F7C7}1.63  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 1291} & UNSAT & \cellcolor[HTML]{C7F7C7}1929  & UNSAT & \cellcolor[HTML]{C7F7C7}11379                                       & UNSAT               & \cellcolor[HTML]{C7F7C7}1.08                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}14066  & \cellcolor[HTML]{C7F7C7}230 & UNSAT & \cellcolor[HTML]{C7F7C7}1.57     & UNK       \\ 
$N_{12}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.21  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 1267} & UNSAT & \cellcolor[HTML]{C7F7C7}2012  & UNSAT & \cellcolor[HTML]{C7F7C7}8629                                       & UNSAT               & \cellcolor[HTML]{C7F7C7}1.13                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}6082   & \cellcolor[HTML]{C7F7C7}78  & UNSAT & \cellcolor[HTML]{C7F7C7}0.98     & UNSAT     \\ 
$N_{13}$                                              & \cellcolor[HTML]{C7F7C7}0.08  & UNK    & \cellcolor[HTML]{C7F7C7}1.56  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 1150} & UNSAT & \cellcolor[HTML]{C7F7C7}956   & UNSAT & \cellcolor[HTML]{C7F7C7}2806                                        & UNSAT               & \cellcolor[HTML]{C7F7C7}0.34                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}4456   & \cellcolor[HTML]{C7F7C7}89  & UNSAT & \cellcolor[HTML]{C7F7C7}1.32     & UNK       \\ 
$N_{14}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.77  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 107}  & UNSAT & \cellcolor[HTML]{C7F7C7}79    & UNSAT & \cellcolor[HTML]{C7F7C7}93                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.18                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}1619   & \cellcolor[HTML]{C7F7C7}18  & UNSAT & \cellcolor[HTML]{C7F7C7}0.63     & UNSAT     \\ 
$N_{15}$                                              & \cellcolor[HTML]{C7F7C7}0.08  & UNK    & \cellcolor[HTML]{C7F7C7}1.11  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 352}  & UNSAT & \cellcolor[HTML]{C7F7C7}299   & UNSAT & \cellcolor[HTML]{C7F7C7}267                                         & UNSAT               & \cellcolor[HTML]{C7F7C7}0.41                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}760    & \cellcolor[HTML]{C7F7C7}11  & UNSAT & \cellcolor[HTML]{C7F7C7}0.77     & UNSAT     \\ 
$N_{16}$                                              & \cellcolor[HTML]{C7F7C7}0.05  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.76  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 219}  & UNSAT & \cellcolor[HTML]{C7F7C7}201   & UNSAT & \cellcolor[HTML]{C7F7C7}82                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.18                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}1105   & \cellcolor[HTML]{C7F7C7}14  & UNSAT & \cellcolor[HTML]{C7F7C7}0.78     & UNSAT     \\ 
$N_{17}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.24  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 1}    & SAT   & \cellcolor[HTML]{C7F7C7}2     & SAT   & \cellcolor[HTML]{C7F7C7}6                                           & SAT                 & \cellcolor[HTML]{C7F7C7}0.02                                      & SAT               & \cellcolor[HTML]{FFFFC7}93     & \cellcolor[HTML]{C7F7C7}2   & SAT   & \cellcolor[HTML]{C7F7C7}0.27     & UNK       \\ 
$N_{18}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.59  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 3}    & SAT   & \cellcolor[HTML]{C7F7C7}2     & SAT   & \cellcolor[HTML]{C7F7C7}6                                           & SAT                 & \cellcolor[HTML]{C7F7C7}0.02                                      & SAT               & \cellcolor[HTML]{FFFFC7}178    & \cellcolor[HTML]{C7F7C7}3   & SAT   & \cellcolor[HTML]{C7F7C7}0.38     & UNK       \\ 
$N_{19}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.28  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 3}    & SAT   & \cellcolor[HTML]{C7F7C7}1     & SAT   & \cellcolor[HTML]{C7F7C7}6                                           & SAT                 & \cellcolor[HTML]{C7F7C7}0.02                                      & SAT               & \cellcolor[HTML]{FFFFC7}44     & \cellcolor[HTML]{C7F7C7}1   & SAT   & \cellcolor[HTML]{C7F7C7}0.22     & UNK       \\ 
$N_{21}$                                              & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}1.00  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 330}  & UNSAT & \cellcolor[HTML]{C7F7C7}239   & UNSAT & \cellcolor[HTML]{C7F7C7}112                                         & UNSAT               & \cellcolor[HTML]{C7F7C7}1.01                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}2678   & \cellcolor[HTML]{C7F7C7}38  & UNSAT & \cellcolor[HTML]{C7F7C7}0.70     & UNSAT     \\ 
$N_{22}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.24  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 415}  & UNSAT & \cellcolor[HTML]{C7F7C7}273   & UNSAT & \cellcolor[HTML]{C7F7C7}210                                         & UNSAT               & \cellcolor[HTML]{C7F7C7}1.85                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}2391   & \cellcolor[HTML]{C7F7C7}32  & UNSAT & \cellcolor[HTML]{C7F7C7}0.95     & UNSAT     \\ 
$N_{23}$                                              & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}0.96  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 243}  & UNSAT & \cellcolor[HTML]{C7F7C7}47    & UNSAT & \cellcolor[HTML]{C7F7C7}35                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.93                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}2357   & \cellcolor[HTML]{C7F7C7}29  & UNSAT & \cellcolor[HTML]{C7F7C7}0.83     & UNSAT     \\ 
$N_{24}$                                              & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}0.84  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 86}   & UNSAT & \cellcolor[HTML]{C7F7C7}23    & UNSAT & \cellcolor[HTML]{C7F7C7}16                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.12                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}2243   & \cellcolor[HTML]{C7F7C7}34  & UNSAT & \cellcolor[HTML]{C7F7C7}0.63     & UNSAT     \\ 
$N_{25}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.75  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 151}  & UNSAT & \cellcolor[HTML]{C7F7C7}95    & UNSAT & \cellcolor[HTML]{C7F7C7}46                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.31                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}265    & \cellcolor[HTML]{C7F7C7}4   & UNSAT & \cellcolor[HTML]{C7F7C7}0.54     & UNSAT     \\ 
$N_{26}$                                              & \cellcolor[HTML]{C7F7C7}0.05  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.59  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 118}  & UNSAT & \cellcolor[HTML]{C7F7C7}71    & UNSAT & \cellcolor[HTML]{C7F7C7}70                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.26                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}166    & \cellcolor[HTML]{C7F7C7}2   & UNSAT & \cellcolor[HTML]{C7F7C7}0.41     & UNSAT     \\ 
$N_{27}$                                              & \cellcolor[HTML]{C7F7C7}0.09  & UNK    & \cellcolor[HTML]{C7F7C7}0.69  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 34}   & UNSAT & \cellcolor[HTML]{C7F7C7}25    & UNSAT & \cellcolor[HTML]{C7F7C7}8                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.04                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}479    & \cellcolor[HTML]{C7F7C7}5   & UNSAT & \cellcolor[HTML]{C7F7C7}0.44     & UNSAT     \\ 
$N_{28}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.44  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 549}  & UNSAT & \cellcolor[HTML]{C7F7C7}121   & UNSAT & \cellcolor[HTML]{C7F7C7}33                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.06                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}421    & \cellcolor[HTML]{C7F7C7}4   & UNSAT & \cellcolor[HTML]{C7F7C7}0.47     & UNSAT     \\ 
$N_{29}$                                              & \cellcolor[HTML]{C7F7C7}0.07  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.20  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 52}   & UNSAT & \cellcolor[HTML]{C7F7C7}6     & UNSAT & \cellcolor[HTML]{C7F7C7}7                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.02                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}16     & \cellcolor[HTML]{C7F7C7}1   & UNSAT & \cellcolor[HTML]{C7F7C7}0.17     & UNSAT     \\ 
$N_{31}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.37  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 478}  & UNSAT & \cellcolor[HTML]{C7F7C7}220   & UNSAT & \cellcolor[HTML]{C7F7C7}283                                         & UNSAT               & \cellcolor[HTML]{C7F7C7}1.12                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}5265   & \cellcolor[HTML]{C7F7C7}81  & UNSAT & \cellcolor[HTML]{C7F7C7}1.01     & UNSAT     \\ 
$N_{32}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.63  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 107}  & UNSAT & \cellcolor[HTML]{C7F7C7}237   & UNSAT & \cellcolor[HTML]{C7F7C7}102                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.44                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}2323   & \cellcolor[HTML]{C7F7C7}48  & UNSAT & \cellcolor[HTML]{C7F7C7}1.27     & UNK       \\ 
$N_{33}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.53  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 116}  & UNSAT & \cellcolor[HTML]{C7F7C7}36    & UNSAT & \cellcolor[HTML]{C7F7C7}12                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.06                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}1903   & \cellcolor[HTML]{C7F7C7}32  & UNSAT & \cellcolor[HTML]{C7F7C7}1.18     & UNSAT     \\ 
$N_{34}$                                              & \cellcolor[HTML]{C7F7C7}0.05  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.84  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 75}   & UNSAT & \cellcolor[HTML]{C7F7C7}32    & UNSAT & \cellcolor[HTML]{C7F7C7}13                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.15                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}1082   & \cellcolor[HTML]{C7F7C7}12  & UNSAT & \cellcolor[HTML]{C7F7C7}0.68     & UNSAT     \\ 
$N_{35}$                                              & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}0.95  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 206}  & UNSAT & \cellcolor[HTML]{C7F7C7}212   & UNSAT & \cellcolor[HTML]{C7F7C7}52                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.91                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}1139   & \cellcolor[HTML]{C7F7C7}14  & UNSAT & \cellcolor[HTML]{C7F7C7}0.63     & UNSAT     \\ 
$N_{36}$                                              & \cellcolor[HTML]{C7F7C7}0.08  & UNK    & \cellcolor[HTML]{C7F7C7}1.57  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 141}  & UNSAT & \cellcolor[HTML]{C7F7C7}50    & UNSAT & \cellcolor[HTML]{C7F7C7}47                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}1.42                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}749    & \cellcolor[HTML]{C7F7C7}13  & UNSAT & \cellcolor[HTML]{C7F7C7}0.96     & UNSAT     \\ 
$N_{37}$                                              & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}0.75  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 304}  & UNSAT & \cellcolor[HTML]{C7F7C7}49    & UNSAT & \cellcolor[HTML]{C7F7C7}10                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.22                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}203    & \cellcolor[HTML]{C7F7C7}3   & UNSAT & \cellcolor[HTML]{C7F7C7}0.55     & UNSAT     \\ 
$N_{38}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.84  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 131}  & UNSAT & \cellcolor[HTML]{C7F7C7}48    & UNSAT & \cellcolor[HTML]{C7F7C7}20                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.23                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}295    & \cellcolor[HTML]{C7F7C7}4   & UNSAT & \cellcolor[HTML]{C7F7C7}0.56     & UNSAT     \\ 
$N_{39}$                                              & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}1.04  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 621}  & UNSAT & \cellcolor[HTML]{C7F7C7}144   & UNSAT & \cellcolor[HTML]{C7F7C7}57                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}1.36                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}657    & \cellcolor[HTML]{C7F7C7}9   & UNSAT & \cellcolor[HTML]{C7F7C7}0.62     & UNSAT     \\ 
$N_{41}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.87  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 49}   & UNSAT & \cellcolor[HTML]{C7F7C7}30    & UNSAT & \cellcolor[HTML]{C7F7C7}40                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}2.73                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}886    & \cellcolor[HTML]{C7F7C7}13  & UNSAT & \cellcolor[HTML]{C7F7C7}0.73     & UNSAT     \\ 
$N_{42}$                                              & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}1.19  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 244}  & UNSAT & \cellcolor[HTML]{C7F7C7}77    & UNSAT & \cellcolor[HTML]{C7F7C7}42                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}1.96                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}6459   & \cellcolor[HTML]{C7F7C7}136 & UNSAT & \cellcolor[HTML]{C7F7C7}1.06     & UNK       \\ 
$N_{43}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.23  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 243}  & UNSAT & \cellcolor[HTML]{C7F7C7}163   & UNSAT & \cellcolor[HTML]{C7F7C7}100                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}1.10                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}3652   & \cellcolor[HTML]{C7F7C7}59  & UNSAT & \cellcolor[HTML]{C7F7C7}0.88     & UNSAT     \\ 
$N_{44}$                                              & \cellcolor[HTML]{C7F7C7}0.05  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.78  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 206}  & UNSAT & \cellcolor[HTML]{C7F7C7}52    & UNSAT & \cellcolor[HTML]{C7F7C7}31                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}1.31                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}338    & \cellcolor[HTML]{C7F7C7}4   & UNSAT & \cellcolor[HTML]{C7F7C7}0.43     & UNSAT     \\ 
$N_{45}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.71  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 217}  & UNSAT & \cellcolor[HTML]{C7F7C7}53    & UNSAT & \cellcolor[HTML]{C7F7C7}32                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}1.49                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}728    & \cellcolor[HTML]{C7F7C7}8   & UNSAT & \cellcolor[HTML]{C7F7C7}0.56     & UNSAT     \\ 
$N_{46}$                                              & \cellcolor[HTML]{C7F7C7}0.07  & UNSAT  & \cellcolor[HTML]{C7F7C7}1.08  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 177}  & UNSAT & \cellcolor[HTML]{C7F7C7}18    & UNSAT & \cellcolor[HTML]{C7F7C7}8                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.02                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}651    & \cellcolor[HTML]{C7F7C7}10  & UNSAT & \cellcolor[HTML]{C7F7C7}0.61     & UNSAT     \\ 
$N_{47}$                                              & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}0.82  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 47}   & UNSAT & \cellcolor[HTML]{C7F7C7}16    & UNSAT & \cellcolor[HTML]{C7F7C7}10                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.17                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}558    & \cellcolor[HTML]{C7F7C7}8   & UNSAT & \cellcolor[HTML]{C7F7C7}0.54     & UNSAT     \\ 
$N_{48}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.58  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 195}  & UNSAT & \cellcolor[HTML]{C7F7C7}68    & UNSAT & \cellcolor[HTML]{C7F7C7}25                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.18                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}218    & \cellcolor[HTML]{C7F7C7}2   & UNSAT & \cellcolor[HTML]{C7F7C7}0.42     & UNSAT     \\ 
$N_{49}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.51  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 422}  & UNSAT & \cellcolor[HTML]{C7F7C7}51    & UNSAT & \cellcolor[HTML]{C7F7C7}19                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.08                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}286    & \cellcolor[HTML]{C7F7C7}4   & UNSAT & \cellcolor[HTML]{C7F7C7}0.28     & UNSAT     \\ 
$N_{51}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.92  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 513}  & UNSAT & \cellcolor[HTML]{C7F7C7}174   & UNSAT & \cellcolor[HTML]{C7F7C7}193                                         & UNSAT               & \cellcolor[HTML]{C7F7C7}2.52                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}931    & \cellcolor[HTML]{C7F7C7}14  & UNSAT & \cellcolor[HTML]{C7F7C7}0.79     & UNSAT     \\ 
$N_{52}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}1.04  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 210}  & UNSAT & \cellcolor[HTML]{C7F7C7}48    & UNSAT & \cellcolor[HTML]{C7F7C7}31                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.86                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}3317   & \cellcolor[HTML]{C7F7C7}55  & UNSAT & \cellcolor[HTML]{C7F7C7}0.76     & UNSAT     \\ 
$N_{53}$                                              & \cellcolor[HTML]{C7F7C7}0.05  & UNK    & \cellcolor[HTML]{C7F7C7}1.29  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 124}  & UNSAT & \cellcolor[HTML]{C7F7C7}39    & UNSAT & \cellcolor[HTML]{C7F7C7}41                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.09                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}3008   & \cellcolor[HTML]{C7F7C7}47  & UNSAT & \cellcolor[HTML]{C7F7C7}0.83     & UNSAT     \\ 
$N_{54}$                                              & \cellcolor[HTML]{C7F7C7}0.07  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.80  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 144}  & UNSAT & \cellcolor[HTML]{C7F7C7}43    & UNSAT & \cellcolor[HTML]{C7F7C7}12                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.12                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}259    & \cellcolor[HTML]{C7F7C7}4   & UNSAT & \cellcolor[HTML]{C7F7C7}0.55     & UNSAT     \\ 
$N_{55}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.36  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 114}  & UNSAT & \cellcolor[HTML]{C7F7C7}61    & UNSAT & \cellcolor[HTML]{C7F7C7}30                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.48                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}209    & \cellcolor[HTML]{C7F7C7}2   & UNSAT & \cellcolor[HTML]{C7F7C7}0.25     & UNSAT     \\ 
$N_{56}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNK    & \cellcolor[HTML]{C7F7C7}0.65  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 160}  & UNSAT & \cellcolor[HTML]{C7F7C7}55    & UNSAT & \cellcolor[HTML]{C7F7C7}45                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.33                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}674    & \cellcolor[HTML]{C7F7C7}8   & UNSAT & \cellcolor[HTML]{C7F7C7}0.43     & UNSAT     \\ 
$N_{57}$                                              & \cellcolor[HTML]{C7F7C7}0.06  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.37  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 38}   & UNSAT & \cellcolor[HTML]{C7F7C7}8     & UNSAT & \cellcolor[HTML]{C7F7C7}8                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.03                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}34     & \cellcolor[HTML]{C7F7C7}1   & UNSAT & \cellcolor[HTML]{C7F7C7}0.31     & UNSAT     \\ 
$N_{58}$                                              & \cellcolor[HTML]{C7F7C7}0.07  & UNK    & \cellcolor[HTML]{C7F7C7}0.89  & UNK    & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 111}  & UNSAT & \cellcolor[HTML]{C7F7C7}48    & UNSAT & \cellcolor[HTML]{C7F7C7}22                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.06                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}1212   & \cellcolor[HTML]{C7F7C7}15  & UNSAT & \cellcolor[HTML]{C7F7C7}0.53     & UNSAT     \\ 
$N_{59}$                                              & \cellcolor[HTML]{C7F7C7}0.04  & UNSAT  & \cellcolor[HTML]{C7F7C7}0.49  & UNSAT  & \cellcolor[HTML]{C7F7C7}{\color[HTML]{000000} 116}  & UNSAT & \cellcolor[HTML]{C7F7C7}57    & UNSAT & \cellcolor[HTML]{C7F7C7}14                                          & UNSAT               & \cellcolor[HTML]{C7F7C7}0.09                                      & UNSAT             & \cellcolor[HTML]{FFFFC7}24     & \cellcolor[HTML]{C7F7C7}1   & UNSAT & \cellcolor[HTML]{C7F7C7}0.33     & UNSAT     \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}


==> preliminary.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
%
%\vspace{-0.25em}

\subsection{Problem definition}

A feed-forward neural network (FNN) consists of an input layer, an output layer, and multiple hidden layers in which each layer is comprised of neurons that are connected to the neurons of preceding layer labeled using weights \cite{hertz1991introduction}. Given an input vector, the output of an FNN is determined by three components: the weight matrices $W_{k,k-1}$, representing the weighted connection between neurons of two consecutive layers $k-1$ and $k$, the bias vectors $b_k$ of each layer, and the activation function $f$ applied at each layer. Mathematically, the output of a neuron $i$ is defined by:
%
\begin{equation*}
y_i = f(\Sigma_{j=1}^n\omega_{ij}x_j + b_i),
\end{equation*}
%
where $x_{j}$ is the $j^{th}$ input of the $i^{th}$ neuron, $\omega_{ij}$ is the weight from the $j^{th}$ input to the $i^{th}$ neuron, $b_i$ is the bias of the $i^{th}$ neuron. In this paper, we are interested in FNN with ReLU activation functions defined by $ReLU(x) = max(0, x)$.
%
%\begin{definition} [Layer Reachable Set] Given a bounded convex polyhedron input set defined as $I \triangleq \{x~|~Ax \leq b, x \in \mathbb{R}^n \}$, the reachable set of a layer $L$ with $m$ neurons corresponding to the input set $I$ is defined by:
  %
%  \begin{equation*}
%       R_{L} \triangleq \{y ~|~y = ReLU(Wx + b),~y \in \mathbb{R}^m, ~x \in I \},
%  \end{equation*}
%  where $W \in \mathbb{R}^{m \times n}$ and $b \in \mathbb{R}^m$ are the weights matrix and bias vector of the layer respectively.
%  %
%\end{definition}
%

\begin{definition}[Reachable Set of FNN]\label{def:reachable set} Given a bounded convex polyhedron input set defined as $\mathcal{I} \triangleq \{x~|~Ax \leq b, x \in \mathbb{R}^n \}$, and an $k$-layers feed-forward neural network $F \triangleq \{L_1, \cdots, L_k\}$, the reachable set $F(\mathcal{I}) = \mathcal{R}_{L_k}$ of the neural network $F$ corresponding to the input set I is defined incrementally by:
  \begin{equation*}
    \begin{split}
      \mathcal{R}_{L_{1}} &\triangleq \{y_1~|~y_1 = ReLU(W_1 x + b_1),~ x \in \mathcal{I}\}, \\
      \mathcal{R}_{L_{2}} &\triangleq \{y_2~|~y_2 = ReLU(W_2 y_1 + b_2),~ y_1 \in \mathcal{R}_{L_1}\}, \\
     &\vdots \\
    \mathcal{R}_{L_k} &\triangleq \{y_k ~|~ y_k = ReLU(W_k y_{k-1} + b_k)\,~y_{k-1} \in \mathcal{R}_{L_{k-1}} \}, \\
    \end{split}
  \end{equation*}
  where $W_k$ and $b_k$ are the weight matrix and bias vector of the $k^{th}$ layer $L_k$. The reachable set $\mathcal{R}_{L_k}$ contains all outputs of the neural network corresponding to all input vectors $x$ in the input set $\mathcal{I}$.

\end{definition}

\begin{definition}[Safety Verification of FNN] Given a $k$-layers feed-forward neural network $F$, and a safety specification $\mathcal{S}$ defined as a set of linear constraints on the neural network outputs $\mathcal{S} \triangleq \{y_k~|~Cy_k \leq d \}$, the neural network $F$ is called to be safe corresponding to the input set $\mathcal{I}$, we write $F(\mathcal{I}) \vDash S$, if and only if $\mathcal{R}_{L_k} \cap \neg \mathcal{S} = \emptyset$, where $\mathcal{R}_{L_k}$ is the reachable set of the neural network with the input set $\mathcal{I}$, and $\neg$ is the symbol for logical negation. Otherwise, the neural network is called to be unsafe $F(\mathcal{I}) \nvDash S$.
\end{definition}


\subsection{Generalized star sets}

\begin{definition}[Generalized Star Set \cite{bak2017simulation}] \label{def:star} A generalized star set (or simply star) $\Theta$ is a tuple $\langle c, V, P \rangle$ where $c \in \mathbb{R}^n$ is the center, $V = \{v_1, v_2, \cdots, v_m\}$ is a set of m vectors in $\mathbb{R}^n$ called basis vectors, and $P: \mathbb{R}^m \to \{ \top, \bot\}$ is a predicate. The basis vectors are arranged to form the star's $n \times m$ basis matrix. The set of states represented by the star is given as:
\begin{equation}
 \llbracket \Theta \rrbracket = \{x~|~x = c + \Sigma_{i=1}^m(\alpha_iv_i)~\text{such that}~P(\alpha_1, \cdots, \alpha_m) = \top \}.
\end{equation}
Sometimes we will refer to both the tuple $\Theta$ and the set of states $\llbracket \Theta \rrbracket$ as $\Theta$. In this work, we restrict the predicates to be a conjunction of linear constraints, $P(\alpha) \triangleq C\alpha \leq d$ where, for $p$ linear constraints, $C \in \mathbb{R}^{p \times m}$, $\alpha$ is the vector of $m$-variables, i.e., $\alpha = [\alpha_1, \cdots, \alpha_m]^T$, and $d \in \mathbb{R}^{p \times 1}$. A star is an empty set if and only if $P(\alpha)$ is empty.
\end{definition}

\begin{proposition} \label{pro1}
  Any bounded convex polyhedron $\mathcal{P} \triangleq \{x~|~Cx \leq d, x \in \mathbb{R}^n \}$ can be represented as a star.
\begin{proof}
    The polyhedron $\mathcal{P}$ is equivalent to the star set $\Theta$ with the center $c = [0, 0, \cdots, 0]^T$, the basic vectors $V = \{e_1, e_2, \cdots, e_n\}$ in which $e_i$ is the $i^{th}$ basic vector of $\mathbb{R}^n$, and the predicate $P(\alpha) \triangleq C\alpha \leq d$.
\end{proof}
\end{proposition}
%
\begin{proposition}[Affine Mapping of a Star]\label{pro2}
Given a star set $\Theta = \langle c, V, P\rangle$, an affine mapping of the star $\Theta$ with the affine mapping matrix $W$ and offset vector $b$ defined by $\bar{\Theta} = \{y~|~y=Wx + b,~x \in \Theta \}$ is another star with the following characteristics.
  \begin{equation*}
    \bar{\Theta} = \langle \bar{c}, \bar{V}, \bar{P} \rangle, ~ \bar{c} = Wc + b, ~\bar{v} = \{Wv_1, Wv_2, \cdots, Wv_m \},~ \bar{P} \equiv P.
  \end{equation*}
  \begin{proof}
    From the definition of a star, we have $\bar{\Theta} = \{y~|~y = Wc + b + \Sigma_{i=1}^m(\alpha_iWv_i),$ such that $~P(\alpha_1, \cdots, \alpha_m) = \top\}$ which implies that $\bar{\Theta}$ is another star with the center $\bar{c} = Wc + b$, basic vectors $\bar{V} =  \{Wv_1, Wv_2, \cdots, Wv_m \}$ and the same predicate $P$ as the original star $\Theta$.
  \end{proof}
\end{proposition}
%
\begin{proposition}[Star and Half-space Intersection]\label{pro:star intersection} The intersection of a star $\Theta \triangleq \langle c, V, P \rangle$ and a half-space $\mathcal{H} \triangleq \{x~|~Hx \leq g \}$ is another star with following characteristics.
  \begin{equation*}
    \begin{split}
      &\bar{\Theta} = \Theta \cap \mathcal{H} = \langle \bar{c}, \bar{V}, \bar{P} \rangle, ~\bar{c} = c,~\bar{V} = V, ~\bar{P} = P \wedge P^{\prime}, \\
      &P^{\prime}(\alpha) \triangleq (H\times V_m) \alpha \leq g - H \times c, V_m = [v_1~v_2 \cdots v_m].
    \end{split}
  \end{equation*}
  \begin{proof}
    For any $x \in \Theta \cap \mathcal{H}$, we have $x = c + \Sigma_{i=1}^m(\alpha_iv_i) \wedge Hx \leq g$, or equivalently, $x = c + \Sigma_{i=1}^m(\alpha_iv_i) \wedge H\times V_m \times \alpha \leq g - H\times c$ which implies that the intersection is another star with the same center $c$ and basic vectors $V$ as $\Theta$, and an updated predicate $\bar{P} = P \wedge P^{\prime}, P^{\prime}(\alpha) \triangleq  H\times V_m \times \alpha \leq g - H\times c$.
  \end{proof}
\end{proposition}


==> reachability_ncs.tex <==
\section{Reachability analysis of neural network control systems with stars}
\vspace{-0.2em}
\seclabel{reachability}
In this section, we extend the star-based reachability algorithm for control systems with neuron network controllers as depicted in Figure \ref{fig:ncs} in which $x(t)$ and $y(t)$ are the state and the output of the nonlinear plant, and $v(t)$ is a reference input. Given a set of initial states of the plant $x(0) \in X(0)$ and the reference input $v(t)$, we are interested in verifying the safety property $\mathcal{S} \triangleq Hx(t) \leq g$ of the closed-loop system in a \emph{continuous bounded time interval} $[0, T]$.

The extended star-based reachability algorithm is given in Algorithm \ref{alg:ncs-reach}, and works as follows. The verification time interval $[0, T]$ is divided uniformly into $N$ equal time steps $\triangle t = t_{k+1} - t_k = T/N$. The zonotope-based reachability algorithm in CORA \ref{xx} is used to compute the reachable set of the plant between two time steps. This algorithm first further divides the time between $t_k$ and $t_{k+1}$ into $N_p$ smaller time steps, and then performs a sound linearization-based reachable set computation for the plant along with $N_p$ time steps to obtain a reachable set with $N_p$ stars. We refer readers to \cite{xx} for the technical details of this approach. The last star in the union is the initial set of states of the plant for the next time interval $[t_{k+1}, t_{k+2}]$. This star is also feedback to the neural network controller (with the output feedback matrix $C$) in combination with the reference input $v(t_{k+1})$ to form a star input set for the controller. Algorithm \ref{alg:ReLU-reach} is invoked to compute the control input $U$ for the next step which is a union of a set of stars. The interval hull of this union is obtained as a unique star control input for the plant. The procedure is performed iteratively until reaching the bounded time interval $T$.
%
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/NCS.pdf}
    \caption{Neural network control system.}
    \label{fig:ncs}
  \end{figure}
  %
\begin{algorithm}[t!]
	\caption{Star-based reachability analysis for neural network control systems}\label{alg:ncs-reach}
	\begin{algorithmic}[1]
		\Input{Plant $P$, initial set $X_0$, output feedback matrix $C$, neural network controller $F$, reference input $v(t)$, uniform sampling step $\triangle t = t_{k+1} - t_k$, number of sampling steps $N$ (verification time $T = N\times \triangle t$), number of time steps for computing the reachable set of the plant $N_p$, i.e., divide $\triangle t$ into $N_p$ time steps}
		\Output{$R$ \% continuous reachable set of the plant, a union of stars}

        \Procedure{\texttt{ $R$ = NcsReach}}{$P, X_0, F, v(t), \triangle t, N$}
		\State $R = \emptyset$
        \State $U = 0$
		\For {\texttt{$i=1:N$}}
		\State $R_1 = P.getReachSet(U, X_0, \triangle t, N_p)$ \% CORA \cite{xx} is invoked to compute $R_1$
        \State $R = R \cup R_1$ \% $R_1$ contains $N_p$ stars
        \State $X_0 = R_1(N_p)$ \% the $N_p^{th}$ star is the initial state for the next step
        \State $\Theta = getStarInput(C * X_0, v(t_i))$ \% feedback $C*X_0$ to the  controller
        \State $U = F(\Theta)$ \% Algorithm \ref{alg:ReLU-reach} is invoked to compute the control input $U$
        \State $U = intervalHull(U)$ \% get a unique star control input set
		\EndFor
		\EndProcedure


	\end{algorithmic}
\end{algorithm}
%

